F2M-Reg: Unsupervised RGB-D Point Cloud Registration with Frame-to-Model Optimization

This work studies the problem of unsupervised RGB-D point cloud registration, which aims at training a robust registration model without ground-truth pose supervision. Existing methods usually leverages unposed RGB-D sequences and adopt a frame-to-frame framework based on differentiable rendering to train the registration model, which enforces the photometric and geometric consistency between the two frames for supervision. However, this frame-to-frame framework is vulnerable to inconsistent factors between different frames, e.g., lighting changes, geometry occlusion, and reflective materials, which leads to suboptimal convergence of the registration model. In this paper, we propose a novel frame-to-model optimization framework named F2M-Reg for unsupervised RGB-D point cloud registration. We leverage the neural implicit field as a global model of the scene and optimize the estimated poses of the frames by registering them to the global model, and the registration model is subsequently trained with the optimized poses. Thanks to the global encoding capability of neural implicit field, our frame-to-model framework is significantly more robust to inconsistent factors between different frames and thus can provide better supervision for the registration model. Besides, we demonstrate that F2M-Reg can be further enhanced by a simplistic synthetic warming-up strategy. To this end, we construct a photorealistic synthetic dataset named Sim-RGBD to initialize the registration model for the frame-to-model optimization on real-world RGB-D sequences. Extensive experiments on four challenging benchmarks have shown that our method surpasses the previous state-of-the-art counterparts by a large margin, especially under scenarios with severe lighting changes and low overlap. Our code and models are available at https://github.com/MrIsland/F2M_Reg.

==> sections/figures/convergence.tex <==
\begin{figure}
\centering
\includegraphics[trim=0.cm 0.3cm 0.1cm 0.2cm, clip, width=\linewidth]{sections/figures/image/convergence2.pdf}

\caption{\textbf{Variation of Inlier Ratio Across Training Epochs.} The pie chart illustrates the distribution of inlier ratios across different ranges, with each range represented by distinct colored blocks. Larger blocks correspond to a higher number of frame pairs that fall within the respective inlier ratio range on the test dataset. This data was obtained by fine-tuning the registration model on 3DMatch and testing it on ScanNet, using frame pairs spaced 50 frames apart.}


\label{fig:convergence}
\end{figure}

==> sections/tables/Ablation_ScanNet_loss.tex <==
\begin{table*}[]
    \centering

    \resizebox{\textwidth}{!}
    {\begin{tabular}{cccccccccccccccccc}
    \toprule
       \multicolumn{1}{c}{\multirow{3}{*}{ Corr }} &
       \multicolumn{1}{c}{\multirow{3}{*}{Circle}}  &
       \multicolumn{1}{c}{\multirow{3}{*}{Train Set}} & \multicolumn{5}{c}{Rotation($^{\circ}$)} & \multicolumn{5}{c}{Translation(cm)} & \multicolumn{5}{c}{Chamfer(mm)} \\
       \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & 
       \multicolumn{1}{c}{} & 
       \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} &  \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} & \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} \\
       \cline{4-18} 
        \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & 5 & 10 & 45 & Mean & Med. & 5 & 10 & 25 & Mean & Med. & 1 & 5 & 10 & Mean & Med. \\
        
    \midrule
         & & & 71.3 & 78.6 & 87.4 & 15.8 & 2.0 & 46.9 & 65.5 & 76.3 & 34.5 & 5.4 & 57.5 & 72.2 & 75.0 & 77.7 & 0.6 \\
        \checkmark & & ScanNet & 71.0 & 77.7 & 86.7 & 18.8 & 2.0 & 48.7 & 66.0 & 75.8 & 34.7 & 5.2 & 58.1 & 72.2 & 75.0 & 83.8 & 0.6 \\
        & \checkmark & ScanNet & 77.1 & 84.3 & \textbf{92.7} & \textbf{10.3} & \textbf{1.9} & 49.1  & 70.2 & 81.6 & \textbf{24.0} & 5.1 & 61.1 & 77.3 & 80.4 & \textbf{62.7} & \textbf{0.5} \\
        \checkmark & \checkmark & ScanNet & \textbf{77.4} & \textbf{84.5} & 92.5 & 15.5 & \textbf{1.9} & \textbf{50.0} & \textbf{70.6} & \textbf{82.1} & 30.1 & \textbf{5.0} & \textbf{61.5} & \textbf{77.6} & \textbf{80.9} & 73.8 & \textbf{0.5}  \\
    \bottomrule
    \end{tabular}}
    \caption{\textbf{Ablation on loss.} \textbf{\textit{Corr}} denotes the correspondence loss. \textbf{\textit{Circle}} denotes the circle loss. All the blank ($1^{\text{st}}$ row) means the registration model was only bootstrapped on the Sim-RGBD dataset without fintuning.}
    \label{tab:Abl_ScanNet_loss}
\end{table*}


==> sections/tables/Ablation_ScanNet_pretraining.tex <==
\begin{table*}[t]
    \centering

    \resizebox{1\linewidth}{!}
    {\begin{tabular}{ccccccccccccccccc}
    \toprule
       \multicolumn{1}{c}{\multirow{3}{*}{ Warm up }} & \multicolumn{1}{c}{\multirow{3}{*}{Train Set}} & \multicolumn{5}{c}{Rotation($^{\circ}$)} & \multicolumn{5}{c}{Translation(cm)} & \multicolumn{5}{c}{Chamfer(mm)} \\
       \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} &  \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} & \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} \\
       \cline{3-17} 
        \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & 5 & 10 & 45 & Mean & Med. & 5 & 10 & 25 & Mean & Med. & 1 & 5 & 10 & Mean & Med. \\
        
    \midrule
        & 3DMatch & 59.0 & 71.3 & 86.3 & 18.6 & 3.5 & 30.4 & 52.3 & 68.0 & 42.2 & 9.2 & 43.2 & 62.1 & 66.5 & 97.0 & 1.6 \\
       \checkmark & 3DMatch & \textbf{72.6} & \textbf{81.1} & \textbf{91.1} & \textbf{12.5} & \textbf{2.2} & \textbf{44.6} & \textbf{65.9} & \textbf{78.5} & \textbf{28.5} & \textbf{5.8} & \textbf{56.1} & \textbf{73.6} & \textbf{77.1} & \textbf{72.0} & \textbf{0.7} \\
    \midrule
        & ScanNet & 74.4 & 82.8 & 92.3 & \textbf{10.8} & 2.1 & 46.8 & 67.9 & 80.4 & \textbf{25.4} & 5.5 & 58.5 & 75.5 & 79.0 & \textbf{67.1} & 0.6 \\
       \checkmark & ScanNet & \textbf{77.4} & \textbf{84.5} & \textbf{92.5} & 15.5 & \textbf{1.9} & \textbf{50.0} & \textbf{70.6} & \textbf{82.1} & 30.1 & \textbf{5.0} & \textbf{61.5} & \textbf{77.6} & \textbf{80.9} & 73.8 & \textbf{0.5}  \\
    \bottomrule
    \end{tabular}}
    \caption{\textbf{Ablation on warming up module.} \textbf{\textit{Warm up}} denotes the process of training the registration model on the Sim-RGBD dataset.}
    \label{tab:Abl_ScanNet_pretrain}
\end{table*}


==> sections/tables/Ablation_ScanNet_rendering.tex <==
\begin{table*}[t]
    \centering
     \resizebox{1\linewidth}{!}
    {\begin{tabular}{lcccccccccccccccc}
    \toprule
       \multicolumn{1}{c}{\multirow{3}{*}{ }} & \multicolumn{1}{c}{\multirow{3}{*}{Train Set}} & \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} &  \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} & \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} \\
       \cline{3-17} 
        \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & 5 & 10 & 45 & Mean & Med. & 5 & 10 & 25 & Mean & Med. & 1 & 5 & 10 & Mean & Med. \\
        
    \midrule
       F2F & ScanNet & 75.2 & 82.5 & 90.3 & \textbf{14.0} & 2.0 & 47.4 & 68.3 & 80.5 & \textbf{30.0} & 5.4 & 58.8 & 76.5 & 79.4 & \textbf{69.2} & 0.6 \\
       F2M & ScanNet & \textbf{77.4} & \textbf{84.5} & \textbf{92.5} & 15.5 & \textbf{1.9} & \textbf{50.0} & \textbf{70.6} & \textbf{82.1} & 30.1 & \textbf{5.0} & \textbf{61.5} & \textbf{77.6} & \textbf{80.9} & 73.8 & \textbf{0.5}  \\
    \bottomrule
    \end{tabular}}
    \caption{\textbf{Ablation on training strategy.} \textbf{\textit{F2F}} refers to the pairwise training strategy of rendering RGB and depth images from the aligned point cloud. \textbf{\textit{F2M}} denotes the training the registration model based on neural rendering approach, where we optimize the input global pose through neural rendering. The optimized pose is then used to guide the supervision of the registration model.}
    \label{tab:Abl_ScanNet_rendering}
\end{table*}


==> sections/tables/Ablation_ScanNet_wo_NeRF.tex <==
\begin{table*}[t]
    \centering

     \resizebox{1\linewidth}{!}
    {\begin{tabular}{cccccccccccccccccc}
    \toprule
       \multicolumn{1}{c}{\multirow{3}{*}{FT}} & \multicolumn{1}{c}{\multirow{3}{*}{$N_{t}$}} & \multicolumn{1}{c}{\multirow{3}{*}{Train Set}} & \multicolumn{5}{c}{Rotation($^{\circ}$)} & \multicolumn{5}{c}{Translation(cm)} & \multicolumn{5}{c}{Chamfer(mm)} \\
       \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} &  \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} & \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} \\
       \cline{4-18} 
        \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & &  5 & 10 & 45 & Mean & Med. & 5 & 10 & 25 & Mean & Med. & 1 & 5 & 10 & Mean & Med. \\
        
    \midrule
        &  &  & 71.3 & 78.6 & 87.4 & 15.8 & 2.0 & 46.9 & 65.5 & 76.3 & 34.5 & 5.4 & 57.5 & 72.2 & 75.0 & 77.7 & 0.6 \\
        \checkmark &   & ScanNet & 76.0 & 84.3 & 92.7 & 10.3 & 2.0 & 46.8 & 69.4 & 81.8 & 23.8 & 5.4 & 59.4 & 77.1 & 80.6 & 61.5 & 0.6 \\
        \checkmark & 20 & ScanNet & 76.7 & 84.4 & \textbf{92.9} & \textbf{10.0} & 1.9 & 48.4 & 69.7 & 81.8 & \textbf{22.7} & 5.2 & 60.7 & 77.1 & 80.2 & \textbf{60.4} & 0.6 \\
        \checkmark & 100 & ScanNet & \textbf{77.4} & \textbf{84.5} & 92.5 & 15.5 & \textbf{1.9} & \textbf{50.0} & \textbf{70.6} & \textbf{82.1} & 30.1 & \textbf{5.0} & \textbf{61.5} & \textbf{77.6} & \textbf{80.9} & 73.8 & \textbf{0.5}  \\
    \bottomrule
    \end{tabular}}
     \caption{\textbf{Ablation on fine-tuning module.} \textbf{\textit{FT}} refers to fine-tuning registration model on the train set, as described in Sec.\ref{sec:method:nerf}. \boldsymbol{$N_{t}$} denotes the number of iterators for tracking. Blanks in the \textbf{\textit{FT}} column indicate that no fine-tuning operation is performed while blanks in the \boldsymbol{$N_{t}$} column signify that no neural implicit field is constructed in those cases. }
    \label{tab:Abl_wo_NeRF}
\end{table*}


==> sections/tables/Convergence_3DMatch_epoch.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}
    {\begin{tabular}{cccccccccccccccccc}
    \toprule
       \multicolumn{1}{c}{\multirow{3}{*}{Epoch}}  &
       \multicolumn{1}{c}{\multirow{3}{*}{Train Set}} & \multicolumn{5}{c}{Rotation($^{\circ}$)} & \multicolumn{5}{c}{Translation(cm)} & \multicolumn{5}{c}{Chamfer(mm)} \\
       \multicolumn{1}{c}{} & 
       \multicolumn{1}{c}{} & 
       \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} &  \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} & \multicolumn{3}{c}{Accuracy $\uparrow$} & \multicolumn{2}{c}{Error$\downarrow$} \\
       \cline{3-17} 
        \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & 5 & 10 & 45 & Mean & Med. & 5 & 10 & 25 & Mean & Med. & 1 & 5 & 10 & Mean & Med. \\
        
    \midrule
         1 & 3DMatch & 71.2 & 79.9 & 90.3 & 13.6 & \underline{2.3} & 42.4 & 63.9 & 77.3 & 30.8 & \underline{6.2} & 54.5 & 72.3 & 75.8 & 75.1 & \underline{0.8} \\
         2 & 3DMatch & 72.6 & 81.1 & 91.1 & 12.5 & \textbf{2.2} & \underline{44.6} & \underline{65.9} & 78.5 & 28.5 & \textbf{5.8} & 56.1 & 73.6 & 77.1 & 72.0 & \textbf{0.7} \\
         3 & 3DMatch & \underline{73.0} & \underline{81.9} & \underline{91.4} & 12.4 & \underline{2.3} & 44.0 & 65.7 & 79.2 & 29.0 & \underline{6.2} & 56.2 & 73.9 & \underline{77.8} & 71.8 & \underline{0.8} \\
         4 & 3DMatch & \textbf{73.5} & \textbf{82.2} & \textbf{91.6} & \textbf{11.9} & \textbf{2.2} & \textbf{44.7} & \textbf{66.4} & \textbf{79.7} & \textbf{26.8} & \textbf{5.8} & \textbf{56.9} & \textbf{74.5} & \textbf{78.2} & \textbf{69.0} & \textbf{0.7} \\
         5 & 3DMatch & \underline{73.0} & 81.7 & \underline{91.4} & \underline{12.2} & 2.4 & 44.5 & \underline{65.9} & \underline{79.4} & \underline{28.2} & 6.4 & \underline{56.6} & \underline{74.0} & 77.7 & \underline{71.5} & \underline{0.8} \\
    \bottomrule
    \end{tabular}}
    \caption{\textbf{Table of performance effects of training different epoch registration. }\textbf{\textit{Epoch}} indicates the number of epochs that the registration model has been trained on 3DMatch. \textbf{Boldfaced} numbers are the best and the second best are \underline{underlined}.}
    \label{tab:Abl_epoch}
\end{table*}

